An information-theoretic lower bound in time-uniform estimation

We present an information-theoretic lower bound for the problem of parameter estimation with time-uniform coverage guarantees. Via a new a reduction to sequential testing, we obtain stronger lower bounds that capture the hardness of the time-uniform setting. In the case of location model estimation, logistic regression, and exponential family models, our $\Omega(\sqrt{n^{-1}\log \log n})$ lower bound is sharp to within constant factors in typical settings.

==> sections/additional-proofs.tex <==
\section{Proof of Lemma~\ref{lemma:kl-cond-bd}}\label{sec:kl-cond-bd}
\begin{proof}
  Let $p, q$ be the densities of $P$ and $Q$ respectively with respect to a
  dominating measure $\mu$.
  Then it is clear that $dP_S/d\mu = \frac{1}{P(S)}p1_S$ and $dQ_S/d\mu = \frac{1}{Q(S)}q1_S$.
  Thus,
  \begin{align*}
    \dkl{P_S}{Q_S}
    &= \int \frac{p}{P(S)}1_S \log\left(\frac{p/P(S)}{q/Q(S)}\right) d\mu \\
    &= \frac{1}{P(S)} \int p\log(p/q)1_S d\mu + \log(Q(S)/P(S)) \\
    &= \frac{1}{P(S)}\dkl{P}{Q} + \log(Q(S)/P(S)) + \frac{1}{P(S)}\int p\log(q/p)1_{S^c}d\mu.
  \end{align*}

  Now, $\log(q/p) = \log(1 + (q-p)/p) \leq (q-p)/p$, and so
  \begin{align*}
    \dkl{P_S}{Q_S}
    &\leq \frac{1}{P(S)}\dkl{P}{Q} + \log(Q(S)/P(S)) + \frac{1}{P(S)}\int (q-p)1_{S^c}d\mu \\
    &= \frac{1}{P(S)}\dkl{P}{Q} + \log(Q(S)/P(S)) + \frac{P(S)-Q(S)}{P(S)}.
  \end{align*}
  Using the same inequality as before, $\log(Q(S)/P(S)) \leq (Q(S)-P(S))/P(S)$,
  and so the latter two terms in the above display are collectively at most 0.
  This proves the claim.
\end{proof}

% \begin{lemma}
%   Let $P_1, \dots, P_M$ be distributions over a set $\cX$ such that
%   $\dkl{P_i}{P_j} \leq D$ for all $i,j \in [M]$.
%   Now let $\correctevent_1, \dots, \correctevent_M$ be measurable sets that partition $\cX$.
%   Then $\max_i P_i(\correctevent_i^c) \geq \frac{M-1}{4}\cdot\exp(-2D)$.
% \end{lemma}
% \begin{proof}
%   Define $\alpha = \max_i P_i(\correctevent_i^c)$.
%   If $\alpha \geq \frac{1}{2}$, then there is nothing to show,
%   so assume otherwise.
%   For any $i \neq j$, we then have by (cite second-order hypercontractive paper Lemma 2.1) that
%   \begin{align*}
%     -\log\left(P_j(\correctevent_i)\right)
%     \leq \frac{\dkl{P_i}{P_j}+\log 2}{1-\alpha}
%     \leq 2(D+\log 2).
%   \end{align*}
%   This implies that $P_j(\correctevent_i) \geq \exp(-2(D+\log 2))$ for all $j \neq i$.
%   Summing over $i$, we thus have
%   \begin{align*}
%     P_j(\correctevent_j^c) = \sum_{i\neq j} P_j(\correctevent_i) \geq (M-1)\exp(-2(D+\log 2)).
%   \end{align*}
% \end{proof}


==> sections/convex-optimization-example.tex <==
\subsection{Convex optimization excess risk}
We take $\Theta = \cX = [0, 1]$,
$\cP$ to be the space of all probability distributions over $\cX$ and
$\ell(\vartheta, x) = |\vartheta - x|$.

We will take $\gamma_k \in [0, 0.5]$ to be a sequence of numbers to be
specified later.
For $v \in \cV$, consider the following random process:
sample $B^v_j \sim \bern(0.5 + (2v_j-1)\gamma_k)$ independently and
let $X^v = 2\sum_{j=1}^\infty B_k 3^{-j}$.
Then take $\distv$ to be the law of $X^v$.

We first compute the distribution closeness.
Let $v, v' \in \cV$ such that $v_{1:k} = v'_{1:k}$.
Then by data-processing inequality and the independence of the $B^v_j$'s,
we have that
\begin{align*}
  \dkl{\distv}{\distvv}
  &\leq \sum_{j=1}^\infty \dkl{B^v_j}{B^{v'}_j}
  &\leq c\sum_{j=1}^\infty \gamma_j^2 \indic{v_j \neq v'_j}
  &\leq c\sum_{j=k+1}^\infty \gamma_j^2.
\end{align*}

\newcommand{\thetamid}{\theta_{\mathsf{mid}}}

Now we compute the parameter separation.
Let $v, v' \in \cV$ such that they differ for the first time at index $k$.
Then consider
$\thetamid = \frac{3}{2} \cdot 3^{-k} + 2\sum_{j=1}^{k-1} v_j\cdot 3^{-j}$.
Taking the derivative of the risk at $\thetamid$, we get
\begin{align*}
  \frac{d}{d\theta}R(\thetamid, \distv)
  &= \distv(\thetamid \geq X^v) - \distv(\thetamid < X^v) \\
  &= 2\P(X^v \leq \thetamid) - 1 \\
  &= 2\P()
\end{align*}


==> sections/kl-location-family.tex <==
\subsection{Proof of Lemma~\ref{lemma:densities-fisher}}
\label{sec:proof-densities-fisher}

We first state the regularity conditions:
we assume that $f$ is twice differentiable, that for suitably small
$\theta > 0$
\begin{align*}
  \int \int_0^\theta \frac{f(x)}{f(x + t)} |f''(x + t)| dt dx <
  \infty, & ~~
  \lim_{t \to 0}
  \int \frac{f(x)}{f(x + t)} f''(x + t) dx
  = \int f''(x) dx, \\
  \mbox{and} & ~~ \lim_{t \to 0}
  \int \frac{f(x)}{f(x + t)}
  \frac{f'(x + t)^2}{f(x + t)} dx
  = \int \frac{f'(x)^2}{f(x)} dx.
\end{align*}
Notably, under these regularity conditions and the existence of the
Fisher information, we have $\int f''(x) dx
= \frac{\partial^2}{\partial t^2} \int f(x + t) dx = 0$.

Now, by Taylor's theorem with remainder, for a twice differentiable $g$ we
have $g(x + \theta) = g(x) + g'(x) \theta + \int_0^\theta g''(x + t) (\theta
- t) dt$, and so letting $g(x) = \log f(x + \theta)$, we have
\begin{equation*}
  \log f(x + \theta)
  = \log f(x) + \frac{f'(x)}{f(x)} \theta
  + \int_0^\theta \left[\frac{f''(x + t)}{f(x + t)}
    - \frac{f'(x + t)^2}{f(x + t)^2}\right] (\theta - t) dt.
\end{equation*}
The shift invariance of the KL means it is equivalent to
show $\dkl{P_0}{P_{-\theta}} = \half I_0 \theta^2 + o(\theta^2)$ for
$\theta$ near 0.
We thus have
\begin{align*}
  \dkl{P_0}{P_{-\theta}}
  & = \int f(x) \log \frac{f(x)}{f(x + \theta)} dx \\
  & = \int f(x)
  \left(\frac{-f'(x)}{f(x)} \theta
  + \int_0^\theta \left[\frac{f'(x + t)^2}{f(x + t)^2}
    - \frac{f''(x + t)}{f(x + t)}\right] (\theta - t) dt \right) dx \\
  & = \int f(x) \int_0^\theta \frac{f'(x + t)^2}{f(x + t)^2}
  (\theta - t) dt dx
  - \int \int_0^\theta \frac{f(x)}{f(x + t)}
  f''(x + t) (\theta - t) dt dx
\end{align*}
because $\int f'(x) dx = 0$.
The first integrand above is nonnegative, so we may switch the order
of integration, yielding
\begin{align*}
  \lefteqn{\int f(x) \int_0^\theta \frac{f'(x + t)^2}{f(x + t)^2} (\theta - t) dt dx} \\
  & = \int_0^\theta \left[\int \frac{f(x)}{f(x + t)}
    \frac{f'(x + t)^2}{f(x + t)}
    dx \right](\theta - t) dt
  =
  \int_0^\theta (I_0 + o(1)) (\theta - t) dt
  = \half I_0 \theta^2 + o(\theta^2)
\end{align*}
as $\theta \to 0$ by the assumed regularity conditions
and because
the Fisher information is constant. Under the assumed
regularity conditions, we may similarly exchange the order
of integration in the second term, and
so defining $r(t) = \int \frac{f(x)}{f(x + t)} f''(x + t) dx$,
we have
\begin{equation*}
  \int \int_0^\theta \frac{f(x)}{f(x + t)}
  f''(x + t) (\theta - t) dt dx
  = \int_0^\theta (\theta - t) r(t) dt.
\end{equation*}
As $r(t) \to 0$ as $t \to 0$ by assumption, this final integral
is $o(\theta^2)$.


==> sections/median-example.tex <==
\subsection{Non-parametric ERM}
We take $\Theta = \cX = [0, 1]$,
$\cP$ to be the space of all probability distributions over $\cX$ and
$\ell(\vartheta, x) = |\vartheta - x|$.
This choice of $\ell$ means we are interested in finding the median of $P$.
To elicit the lower bound, we will construct a sub-family
$\{P_v\}_{v \in \cV} \subset \cP$ such that
\begin{align*}
  \delta_k \geq c \cdot 5^{-2k}
  \qquad\mathrm{and}\qquad
  \Delta_k \leq 2 \log 3 \cdot 5^{-k}.
\end{align*}
Assuming for the moment that such a sub-family exists, we get from
Corollary~\ref{cor:est-lb} that by taking $n_k = \inf\{n : t(n) < 9\cdot 5^{-k}/8\}$,
\begin{align*}
  n_k \geq \frac{1-\alpha}{2\log 3}5^k.
\end{align*}
Then, by arguing identically as in Section~\ref{sec:loc-models}, we get that
\begin{align*}
  t(n) \geq c_1 \sqrt{\frac{(1-\alpha)\log\log n}{n}},
\end{align*}
infinitely often.

We now construct $\{P_v\}$.
First consider the function
\begin{align*}
  q(x)
  &= \begin{cases}
    2 & x \in [0, 0.2) \\
    0 & x \in [0.2, 0.4) \\
    \tfrac{2}{3} & x \in [0.4, 1]
  \end{cases}.
\end{align*}

\shnote{maybe add a figure}

Notice that $\int_0^1 q = 0.8$.
We define $a_{v, k} = \sum_{j=1}^k (2v_j + 1) 5^{-j}$
% and the functions
% $q_{v, k}$ will be such that they vanish on $[a_{v, k}, a_{v, k} + 5^{-k}]$
% and non-zero elsewhere on $[0, 1]$.
and define functions $q_{v, k} : [0, 1] \rightarrow \R_+$ for $k \geq 1$ as
\begin{align*}
  q_{v, k}(x)
  &=
  \begin{cases}
    q(5^{k-1}(x-a_{v, k-1})) & v_{k} = 0 \\
    q(1-5^{k-1}(x-a_{v, k-1})) & v_{k} = 1,
  \end{cases}
\end{align*}
where $q(\cdot)$ is taken to be $0$ for arguments outside $[0, 1]$.
Because $\int_0^1 q_{v, k} = 2 \cdot 5^{-k}$, we can take $P_v$ to be the
distribution with density $p_v = \sum_{k=1}^\infty q_{v, k}$.

We now show that $P_v$ has unique median
$a_v = \lim_{k \rightarrow \infty} a_{v, k}$.
We begin by analyzing the support of $q_{v, k}$.
If $v_k = 0$, we see by the definition of $q$ that
\begin{align*}
  \supp q_{v, k}
  &= [a_{v, k-1}, a_{v, k-1} + 5^{-k})
    \cup [a_{v, k-1} + 2 \cdot 5^{-k}, a_{v, k-1} + 5^{1-k}] \\
  &= [a_{v, k-1}, a_{v, k})
  \cup [a_{v, k} + 5^{-k}, a_{v, k} + a_{v, k-1} + 5^{1-k}] \\
  &= [a_{v, k-1}, a_{v, k-1} + 5^{1-k}] \setminus [a_{v, k}, a_{v, k} + 5^{-k}).
\end{align*}
Similar calculations will show that
$\supp q_{v, k}
= [a_{v, k-1}, a_{v, k-1} + 5^{1-k}] \setminus [a_{v, k}, a_{v, k} + 5^{-k})$
if $v_k = 1$.
Thus, the supports of $q_{v, k}$ are pairwise disjoint and support almost all
$x \in [0, 1]$.
This implies $p_v$ is supported on almost all of $[0, 1]$.
Because $p_v \geq \tfrac{2}{3}$ on its support, we have can thus conclude
that it has a unique median $m_v$.
Moreover,
\begin{align*}
  \frac{d^2}{d\theta^2} R(\theta, \distv)
  &= \frac{d}{d\theta} (\distv(X \leq \theta) - \distv(X \geq \theta))
  = 2p_v(\theta)
  \geq \frac{4}{3},
\end{align*}
which implies that $R(\theta, \distv) \geq \frac{2}{3}(\theta - m_v)^2$.

Now we see that $m_v = a_v$ by the following computation:
\begin{align*}
  \int_0^{a_v} q_{v, k}
  = ...
\end{align*}

We now compute the parameter separation of $\{P_v\}$.
Let $v, v' \in \cV$ be such that $v_{1:k} \neq v'_{1:k}$ and take without loss
of generality that $k$ is the index where $v, v'$ first differ.
Then,
\begin{align*}
  |a_v - a_{v'}| 
  &= \left| \sum_{j=1}^\infty (2(v_j - v'_j) + 1) 5^{-j} \right|
  \geq 3 \cdot 5^{-k} - \left| \sum_{j=k+1}^\infty (2(v_j - v'_j) + 1) 5^{-j} \right|
  \geq \frac{9}{4} \cdot 5^{-k}.
\end{align*}
Combining this with the growth rate of the risk, we have for any $\theta$ that
$R(\theta, \distv) + R(\theta, \distvv) \geq c 5^{-2k}$, for some numerical
constant $c$.

Now we compute the distribution closeness of $\{P_v\}$.
Let $v, v' \in \cV$ such that $v_{1:k-1} = v'_{1:k-1}$.
Note that $a_{v, j} = a_{v', j}$ for all $j \leq k-1$, and so
$p_v(x) = p_{v'}(x)$ for all $x \in [a_{v, k-1}, a_{v, k-1} + 5^{-k}]^c$.
Furthermore, because $\frac{2}{3} \leq p_v(x) \leq 2$ for all $x$, we also have
that $|\log (p_v(x)/p_{v'}(x))| \leq \log 3$ for all $x$. Hence,
\begin{align*}
  \dkl{\distv}{\distvv}
  &= \int_0^1 p_v \log\left(\frac{p_v}{p_{v'}}\right) \\
  &= \int_{a_{v, k-1}}^{a_{v, k-1} + 5^{-k}} p_v \log\left(\frac{p_v}{p_{v'}}\right) \\
  &\leq \int_{a_{v, k-1}}^{a_{v, k-1} + 5^{-k}} 2 \log 3 \\
  &= 2 \log 3 \cdot 5^{-k}
\end{align*}


==> sections/setup.tex <==
\section{Problem Setup}
Let $\cP$ be a family of distributions over a domain $\cX$,
let $\Theta \subset \R$ be a parameter space, and let
$\ell : \Theta \times \cX \rightarrow \R_+$ be a loss function that is convex
in its first argument.
We are interested finding estimators that minimize the population loss:
\begin{align*}
  \theta(P)
  := \argmin_{\vartheta \in \Theta}  \left\{
    L(\vartheta, P) := \E_{X \sim P}[\ell(\vartheta, X)]
  \right\}.
\end{align*}
We measure the error of the estimator through the excess risk
$R(\theta, P) = L(\theta, P) - L(\theta(P), P)$.

We assume that that the model observes $X_1, X_2, \dots \simiid P$ and at every
step $n \in \N$, returns an estimate $\hat{\theta}_n$ based on the first
$n$ samples.
We use $\P_P$ to denote the probability space generated by $P$ over the
random variables $X_1, X_2, \dots$.

\begin{definition}[$(\alpha, t(\cdot))$-time-uniform
    estimator]\label{def:t-unif-est}
  A sequence of estimators $\hat{\theta} = (\hat{\theta}_n)_{n \in \N}$ is an
  \textit{$(\alpha, t(\cdot))$-time-uniform estimator} if the following hold:
  \begin{enumerate}
    \item (measurability) $\hat{\theta}_n \in m(X_{1:n})$ and
    \item (time-uniform utility) for all $P \in \cP$,
          $\P_P(R(\hat{\theta}_n, P) \leq t(n), \forall n \in \N) \geq 1-\alpha$.
  \end{enumerate}
\end{definition}

Our lower bound strategy will be to find a maximum rate of decay that $t(\cdot)$
must satisfy infinitely often for there to exist an
$(\alpha, t(\cdot))$-time-uniform estimator.
% To do so, we proceed in the next section by reducing the estimation problem to 
% a related testing problem.

\begin{remark}
  In Definition~\ref{def:t-unif-est}, the measurability condition disallows
  randomized estimators.
  However, we can remedy this by augmenting the problem setup by taking
  $\tilde{X} = \cX \times \Omega$ and
  $\tilde{\cP} = \{P \otimes U \mid P \in \cP\}$, where $\Omega$ is some
  domain and $U$ is some distribution on $\Omega$.
  We similarly modify the loss as $\tilde{\ell}(\theta, (x, \omega)) = \ell(\theta, x)$,
  which preserves the population ERM function.
  After we do this augmentation, the estimator now has access to random noise
  at each step $n$ and so it no longer needs to depend deterministically on the
  samples from $P$.
  We still need to justify that the problem does not become information-theoretically
  easier as a result of this augmentation, but we defer that until after
  we introduce the information quantity.
\end{remark}

